Branching Processes for QuickCheck Generators

In QuickCheck (or, more generally, random testing), it is challenging to control random data generators' distributions---specially when it comes to user-defined algebraic data types (ADT). In this paper, we adapt results from an area of mathematics known as branching processes, and show how they help to analytically predict (at compile-time) the expected number of generated constructors, even in the presence of mutually recursive or composite ADTs. Using our probabilistic formulas, we design heuristics capable of automatically adjusting probabilities in order to synthesize generators which distributions are aligned with users' demands. We provide a Haskell implementation of our mechanism in a tool called DRaGeN and perform case studies with real-world applications. When generating random values, our synthesized QuickCheck generators show improvements in code coverage when compared with those automatically derived by state-of-the-art tools.

==> Makefile <==
MAIN = main.tex
LHS2TEX = false
PDF = pdf

ifeq ($(PDF),pdf)
FIGEXT    = pdf
OUTEXT    = pdf
else
FIGEXT    = eps
OUTEXT    = dvi
endif

BASE      := $(basename $(MAIN))
SRCEXT    := $(patsubst $(BASE).%,%,$(MAIN))
XFIGS     := $(wildcard *.fig)
DIAFIGS   := $(wildcard *.dia)
SVGFIGS   := $(wildcard *.svg)
TEXFIGS   := $(XFIGS:.fig=.tex) # $(DIAFIGS:.dia=.tex)
BINFIGS   := $(XFIGS:.fig=.$(FIGEXT)) $(DIAFIGS:.dia=.$(FIGEXT)) $(SVGFIGS:.svg=.$(FIGEXT)) $(GENFIGS)
STYLINK	  := $(notdir $(wildcard ../*.sty))
STYFILES  := $(sort $(STYLINK) $(wildcard *.sty))
TEXFILES  := $(sort $(MAIN) $(wildcard *.tex) $(STYFILES) $(TEXFIGS))
BIBFILES  := $(wildcard *.bib)

JGRAPHS   := $(wildcard *.j)
GGRAPHS   := $(wildcard *.gnuplot)
GRAPHS    := $(JGRAPHS.j=.$(FIGEXT)) $(GGRAPHS:.gnuplot=.$(FIGEXT))

ifeq ($(PDF),pdf)
IMAGESRC  := $(wildcard figs/*.gif) $(wildcard figs/*.eps)
else
IMAGESRC  := $(wildcard figs/*.gif)
endif
IMAGEGEN  := $(addsuffix .$(FIGEXT), $(basename $(IMAGESRC)))
IMAGES    := $(sort $(IMAGEGEN) $(wildcard figs/*.$(FIGEXT)))
IMAGEDIST := $(filter-out $(IMAGEGEN), $(IMAGES)) \
		$(wildcard figs/*.odp) $(wildcard figs/*.ppt)

ifeq ($(PDF),pdf)
LATEX     = pdflatex \\nonstopmode\\input
else
LATEX     = latex
#\\nonstopmode\\input
DVIPS     = dvips -j0 -G0 -t letter -Pdownload35
PS2PDF    = GS_OPTIONS=-sPAPERSIZE=letter ps2pdf -sPAPERSIZE=letter -dEmbedAllFonts=true
#PS2PDF    = ps2pdf
endif
BIBTEX    = bibtex -min-crossrefs=1000

all: $(BASE).pdf

ifeq ($(LHS2TEX),true)
LHS2TEXOUT  = $(MAIN)
LHS2TEXDEPS = $(wildcard $(shell egrep '%include .*.(tex|ltx)' $(BASE).lhs.$(SRCEXT) | cut -d ' ' -f 2 | xargs))
$(MAIN): $(BASE).lhs.$(SRCEXT) $(TEXFILES) $(LHS2TEXDEPS)
	lhs2TeX  $(BASE).lhs.$(SRCEXT) > $(MAIN)
else
LHS2TEXOUT  =
endif

ifeq ($(PDF),pdf)
%.pdf %.tex: %.fig
	fig2dev -L pdftex -p1 $< > $*.pdf
	fig2dev -L pdftex_t -p $*.pdf $< > $*.tex

%.pdf: %.eps
	perl -ne 'exit 1 unless /\n/' $< \
		|| perl -p -i -e 's/\r/\n/g' $<
	epstopdf --outfile=$@ $<

figs/%.pdf: figs/%.gif
	convert $< $@

%.ps: %.pdf
	pdftops -paper A4 $< $@

else
%.ps: %.dvi
	$(DVIPS) $< -o $@

%.eps %.tex: %.fig
	fig2dev -L pstex -p1 $< > $*.eps
	fig2dev -L pstex_t -p $*.eps $< > $*.tex
endif

%.eps: %.dia
	unset DISPLAY; dia -n -e $@ $<
%.tex: %.dia
	unset DISPLAY; dia -n -e $@ $<
%.eps: %.j
	@rm -f $@~
	jgraph $< > $@~
	mv -f $@~ $@
%.eps: %.gnuplot %.data
	gnuplot $*.gnuplot
%.pdf: %.svg
	inkscape -z -A $@ $< && cp $@ .missing/$@ || cp .missing/$@ $@

$(STYLINK):
	rm -f $@
	ln -s ../$@ .

RERUN = egrep -q '(^LaTeX Warning:|\(natbib\)).* Rerun' $*.log
UNDEFINED = egrep -q '^(LaTeX|Package natbib) Warning:.* undefined' $*.log

# So you can "setenv ALWAYS yes" instead of butchering the Makefile...
ifneq ($(ALWAYS),)
ALWAYS = always
endif
$(BASE).$(OUTEXT): %.$(OUTEXT): %.$(SRCEXT) $(TEXFILES) $(BIBFILES) \
				$(BINFIGS) $(GRAPHS) $(IMAGES) $(ALWAYS)
	test ! -s $*.aux || $(BIBTEX) $* || rm -f $*.aux $*.bbl
	$(LATEX) $< || ! rm -f $@
	if $(UNDEFINED); then \
		$(BIBTEX) $* && $(LATEX) $< || ! rm -f $*.bbl $@; \
	fi
	! $(RERUN) || $(LATEX) $< || ! rm -f $@
	! $(RERUN) || $(LATEX) $< || ! rm -f $@
ifeq ($(PDF),pdf)
	touch $*.dvi
	test ! -f .xpdf-running || xpdf -remote $(BASE)-server -reload
else
$(BASE).pdf: %.pdf: %.ps
	$(PS2PDF) $< $@
	test ! -f .xpdf-running || xpdf -remote $(BASE)-server -reload
endif

DIST = GNUmakefile $(filter-out $(TEXFIGS), $(TEXFILES)) \
	$(XFIGS) $(DIAFIGS) $(SVGFIGS) $(GENFIGSRC) \
	$(JGRAPHS) $(GGRAPHS) $(GGRAPHS:.gnuplot=:.data) \
	$(IMAGESRC) $(IMAGEDIST) $(BIBFILES)
dist: $(BASE).tar.gz
$(BASE).tar.gz: $(DIST)
	tar -chzf $@ -C .. \
		$(patsubst %, $(notdir $(PWD))/%, $(DIST))

PREVIEW := $(BASE)
preview: $(PREVIEW).pdf
	if test -f .xpdf-running; then			\
		xpdf -remote $(BASE)-server -quit;	\
		sleep 1;				\
	fi
	touch .xpdf-running
	(xpdf -remote $(BASE)-server $(PREVIEW).pdf; rm -f .xpdf-running) &

show: $(BASE).pdf
	xpdf -fullscreen $(BASE).pdf

osx: $(BASE).pdf
	open $(BASE).pdf

check:
	pdflatex $(BASE).ltx | grep -e "multiply" -e "undefined"

EXTRAIGNORE = '*~' '*.aux' '*.bbl' '*.blg' '*.log' '*.dvi' '*.bak' '*.out'
ignore:
	rm -f .gitignore
	(for file in $(EXTRAIGNORE); do \
		echo "$$file"; \
	done; \
	for file in .xpdf-running \
			$(BASE).tar.gz \
			$(TEXFIGS) $(BINFIGS) $(GRAPHS) $(IMAGEGEN) \
			$(BASE).ps $(BASE).pdf; do \
		echo "/$$file"; \
	done) | sort > .gitignore
	git add .gitignore

clean:
	rm -f $(BASE).ps $(BASE).pdf $(BASE).tar.gz
	rm -f $(TEXFIGS) $(GRAPHS) $(IMAGEGEN)
	rm -f $(LHS2TEXOUT)
	rm -f *.dvi *.aux *.log *.bbl *.blg *.lof *.lot *.toc *.bak *.out
	rm -f *~ *.core core

binfigsclean: clean
	rm -f $(BINFIGS)

always:
	@:

.PHONY: install clean binfigsclean all always ignore preview show osx dist

spell:
	make clean
	for i in $(wildcard *.tex); do aspell -p ./aspell.words -c $$i; done

flat:
	./flatten.pl $(MAIN) > $(BASE)-flat.tex

proof:
	./weasel *.tex
	./passive *.tex

